SoK: Decentralized Exchanges (DEX) with Automated Market Maker (AMM) Protocols

As an integral part of the decentralized finance (DeFi) ecosystem, decentralized exchanges (DEXs) with automated market maker (AMM) protocols have gained massive traction with the recently revived interest in blockchain and distributed ledger technology (DLT) in general. Instead of matching the buy and sell sides, automated market makers (AMMs) employ a peer-to-pool method and determine asset price algorithmically through a so-called conservation function. To facilitate the improvement and development of automated market maker (AMM)-based decentralized exchanges (DEXs), we create the first systematization of knowledge in this area. We first establish a general automated market maker (AMM) framework describing the economics and formalizing the system's state-space representation. We then employ our framework to systematically compare the top automated market maker (AMM) protocols' mechanics, illustrating their conservation functions, as well as slippage and divergence loss functions. We further discuss security and privacy concerns, how they are enabled by automated market maker (AMM)-based decentralized exchanges (DEXs)' inherent properties, and explore mitigating solutions. Finally, we conduct a comprehensive literature review on related work covering both decentralized finance (DeFi) and conventional market microstructure.

==> backup/comparison_backup.tex <==
\input{exhibits/comparison_table}

\section{Comparison of AMM protocols}
\label{sec:comp}

AMM-based DEXs are home to billions of dollars worth of on-chain liquidity. \autoref{tab:comparison} list major AMM protocols, their respective value locked, as well as some other general metrics. Uniswap is undeniably the biggest AMM measured by trade volume, as confirmed by the volume growth displayed in \autoref{fig:uniswap_vol_poolcount}, and the number of governance token holders, although it is remarkable that Sushiswap has more value locked within the protocol. The number of governance token holders of smaller protocols as Bancor and Balancer are relatively big compared to Curve token holders, as they do approximately half of the volume but have 25 to 50\% more governance token holders. \autoref{fig:pooltimeseries} shows an increasing trend over all prominent AMMs. Note that the volumes of March 2021 are not complete yet. While Curve only has 17 pools at the moment of writing, Uniswap has over 30,000. DODO is relatively new, but already showcases around 200\% growth compared to the start of 2021 in terms of volume.

For the rest of this section, we focus on the four most representative ones: Uniswap v2, Balancer v1, Curve, and DODO. We describe the liquidity pool structures of those protocols, and subsequently derive and illustrate the conservation function, slippage, as well as divergence loss of those protocol in \autoref{fig:consfunc}, \autoref{fig:slippage} and \autoref{fig:divloss}, respectively. For denominating purposes, we always use token$_1$ as price or value unit; namely, token$_1$ is the assumed numéraire.

\input{exhibits/volume_poolcount}

\subsection{Uniswap V2}

\subsubsection{Pool structure}

The Uniswap protocol prescribes that a liquidity pool always consists of one pair of assets. The pool smart contract always assumes that the reserves of the two assets have equal value.

\subsubsection{Formulas}

\paragraph{Conservation function}

Uniswap implements a conservation function with constant-product invariant (\autoref{fig:unicons}). Specifically, the product of reserve quantity of token$_1$, $r_1$, and reserve quantity of token$_2$, $r_2$, stays constant with swapping:
\begin{align}
  \label{eq:unicons}
  \const = r_1 \cdot r_2
\end{align}

\paragraph{Spot exchange rate}

Given the {\em equal value assumption} encoded in the pool smart contract, the implied spot price of assets in a liquidity pool can be derived based on the ratio between their reserve quantities. Specifically, denominated in token~1, the price of token$_2$ can be expressed as:
\begin{align}
  \label{eq:uniswapprice}
  {_1E_2} = \frac{r_1}{r_2}
\end{align}

\paragraph{Swap amount}
Based on the Uniswap conservation function (\autoref{eq:unicons}), the amount of token$_2$ received $x_2$ (spent when $x_2<0$) given amount of token$_1$ spent $x_1$ (received when $x_1<0$) can be calculated following the steps described in \autoref{sec:form_sa}:
\begin{align}
  \label{eq:uniswapinput}
  r'_1 &
  % \coloneqq R_1(x_1) 
  = r_1 + x_1
  \nonumber \\
  r'_2 &
  % \coloneqq R_2(x_1)
  = \frac{\const}{r'_1}
  \nonumber \\
  x_2  &
  % \coloneqq X_2(x_1) 
  = r_2 - r'_2
\end{align}



% \subparagraph{Input given output}

% \begin{align}
% x_2 &= r_2 - r'_2
% \\
% r'_2 &= \frac{\const}{r'_2}
% \\
% x_1 &= r'_1 - r_1
% \label{eq:uniswapoutput}
% \end{align}


\paragraph{Slippage}
The slippage that a Uniswap user experiences when swapping $x_1$ token$_1$ with $x_2$ token$_2$ can be expressed as:
\begin{align}
  S(x_1) = \frac{x_1/x_2}{{_1E_2}} -1 = \frac{x_1}{r_1}
  \label{eq:uniswapslippage}
\end{align}

\autoref{fig:uniswapslippage} illustrates the relationship between Uniswap slippage and normalized token$_1$ reserve change $\frac{x_1}{r_1}$.

\paragraph{Divergence loss}
\label{sec:univ2div}
Given the equal value assumption with Uniswap, the reserve value of token~1, $V_1$, equals exactly half of original value of the entire pool $V$ (token$_1$ being numéraire):
\begin{align}
  \frac{V}{2} & = V_1 = V_2 = r_1
\end{align}


Should a liquidity provider have held $r_1$ token$_1$ and $r_2$ token$_2$, then when token$_2$ appreciates by $\rho$ (depreciates when $\rho<0$), the total value of the original reserve composition $V_\text{held}$ becomes:
\begin{align}
  V_\text{held} & = V + V_2 \cdot \rho = r_1 \cdot (2+\rho)
\end{align}

With $r_1$ token$_1$ and $r_2$ token$_2$ locked in a liquidity pool from the beginning, their quantity ratio would have been updated through users' swapping to result in token$_2$'s price change of $\rho$. The equal value assumption still holds, and the updated pool value $V'$ becomes:
\begin{align}
  \frac{V'}{2} & = V'_1  = V'_2 = r'_1 = r_1 \cdot \sqrt{1+ \rho}
\end{align}

Note that $r'_2  = \frac{r_2}{\sqrt{1+ \rho}}$ and $p' = \frac{(1+\rho) r_1}{r_2}$, which preserves the invariance of $\const$, and reflects the change in token$_2$'s spot exchange rate against token$_1$.

As illustrated in \autoref{fig:unicons}, the divergence loss due to liquidity provision as opposed of holding can thus be expressed as a function of price change:
\begin{align}
  L(\rho) & = \frac{V'}{V_\text{held}} -1 = \frac{\sqrt{1+\rho}}{1+\frac{\rho}{2}} -1
  \label{eq:unidiv}
\end{align}

\subsection{Uniswap V3}

Uniswap V3 is the next generation version of Uniswap V2 where liquidity providers can concentrate their liquidity on a fraction of the bonding curve, thus virtually amplifying the conservation function invariant and consequently reducing the slippage.

Suppose a liquidity provider supplies $\revision{\mathcal{R}_1}$ token$_1$ and $\revision{\mathcal{R}_2}$ token$_2$, with the restriction that his liquidity is only used for a specific range of exchange rates: $[\frac{\revision{\mathcal{R}_1}}{\revision{\mathcal{R}_2} \cdot \mathcal{A}}, \frac{\revision{\mathcal{R}_1} \cdot \mathcal{A}}{\revision{\mathcal{R}_2}}]$ where $\mathcal{A} > 1$ and the initial exchange rate equals $\frac{\revision{\mathcal{R}_1}}{\revision{\mathcal{R}_2}}$.
The shape of the conservation function is then {\em identical} to liquidity provision of the following amounts under Uniswap V2:
\begin{align}
  r_1^\text{equiv} = \frac{\revision{\mathcal{R}_1}}{1-\frac{1}{\sqrt{\mathcal{A}}}} \\
  r_2^\text{equiv} = \frac{\revision{\mathcal{R}_2}}{1-\frac{1}{\sqrt{\mathcal{A}}}}
\end{align}

\subsubsection{Conservation function}

The bonding curve of a Uniswap V3 pool is equivalent to that of a Uniswap V2 one moving left along the x-axis by $(r_1^\text{equiv} - \revision{\mathcal{R}_1})$ and down along the y-axis by $(r_2^\text{equiv} - \revision{\mathcal{R}_2})$. Thus, Uniswap V3 conservation function can be expressed as:
\begin{align}
  \label{eq:uniswapv3cons}
  [r_1 + (r_1^\text{equiv} - \revision{\mathcal{R}_1})] \cdot
  [r_2 + (r_2^\text{equiv} - \revision{\mathcal{R}_2})] = r_1^\text{equiv} \cdot r_2^\text{equiv}
  \nonumber \\
  \left(
  r_1 + \frac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  \right) \cdot
  \left(
  r_2 + \frac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1}
  \right) = \frac{
    \mathcal{A} \cdot \revision{\mathcal{R}_1} \cdot \revision{\mathcal{R}_2}}{(\sqrt{\mathcal{A}} -1)^2}
\end{align}
where $0 \leq r_1 \leq \revision{\mathcal{R}_1} \cdot (\sqrt{A} + 1)$ and $0 \leq r_2 \leq \revision{\mathcal{R}_2} \cdot (\sqrt{A} + 1)$.

\subsubsection{Exchange rate}

\begin{align}
  \label{eq:uniswapv3ex}
  {}_1E_2 = \frac{
    r_1 + \frac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  }{
    r_2 + \frac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1}
  }
\end{align}

Note that when token$_1$ is depleted, i.e. $r_1 = 0$, then
\begin{align}
  r_2 + \tfrac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1} = \tfrac{\mathcal{A} \cdot \revision{\mathcal{R}_2}}{
    \sqrt{\mathcal{A}} -1
  }
  \nonumber \\
  {}_1E_2 = \tfrac{\revision{\mathcal{R}_1}}{\revision{\mathcal{R}_2} \cdot \mathcal{A}
  }
  \nonumber
\end{align}
Similarly, when token$_2$ is depleted, i.e. $r_2 = 0$, then ${}_1E_2 =  \frac{\revision{\mathcal{R}_1}}{\revision{\mathcal{R}_2}
    \cdot \mathcal{A}}$

\subsubsection{Swap amount} The swap amount can be derived from the conservation function \autoref{eq:uniswapv3cons}:
\begin{align}
  \label{eq:uniswapv3input}
  r'_1 &
  % \coloneqq R_1(x_1) 
  = r_1 + x_1
  \nonumber \\
  r'_2 &
  % \coloneqq R_2(x_1)
  =
  \tfrac{\revision{\mathcal{R}_1} \revision{\mathcal{R}_2}}{(1-\frac{1}{\sqrt{\mathcal{A}}})^2} \Big/
  \left(
  r'_1 + \tfrac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  \right) - \tfrac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1}
  \nonumber \\
  x_2  &
  % \coloneqq X_2(x_1) 
  = r_2 - r'_2
\end{align}

% Note that to ensure $r'_1, r'_2 \geq 0$, $-r_1 \leq x_1 \leq \revision{\mathcal{R}_1} - r_1$

\subsubsection{Slippage} The slippage should have the same magnitude as in Uniswap V2, but with $r_1$ amplified by an increase of $\frac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}$:
% i think it moght depend
\begin{align}
  S(x_1) = \frac{x_1/x_2}{{_1E_2}} -1 = \frac{x_1}{r_1 +  \frac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  }
  \label{eq:uniswapv3slippage}
\end{align}


\subsubsection{Divergence loss}
Using the intermediary results from \autoref{sec:univ2div}, we can easily derive $V_\text{held}$, $r_1'$ and $r_2'$, and subsequently $V'$:
\begin{align}
  V_\text{held} & = C_1 \cdot (2+\rho)
  \\
  r'_1          & = r_1^\text{equiv}
  \sqrt{1+\rho}
  - \tfrac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  = \tfrac{\revision{\mathcal{R}_1} \cdot (\sqrt{1+\rho} -
    \frac{1}{\sqrt{\mathcal{A}}})
  }{1-\frac{1}{\sqrt{\mathcal{A}}}}
  \nonumber                                                                                                                                            \\
  r'_2          & = \tfrac{r_2^\text{equiv}}{\sqrt{1+\rho}}
  - \tfrac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1}
  =
  \tfrac{ \revision{\mathcal{R}_2}
    (
    \frac{1}{\sqrt{1+\rho}} -\frac{1}{\sqrt{\mathcal{A}}}
    )
  }{
    1-\frac{1}{\sqrt{\mathcal{A}}}
  }
  \nonumber                                                                                                                                            \\
  V'            & = V_1' + V_2' = r_1' + \tfrac{\revision{\mathcal{R}_1} (1+\rho) r'_2}{\revision{\mathcal{R}_2}} = \tfrac{ \revision{\mathcal{R}_1} (
    2 \sqrt{1+\rho} - \frac{2+\rho}{\sqrt{\mathcal{A}}}
    )
  }{1-\frac{1}{\sqrt{\mathcal{A}}}}
  % V_1' & = r_1^\text{equiv}
  % \sqrt{1+\rho}
  % - \frac{\revision{\mathcal{R}_1}}{\sqrt{\mathcal{A}}-1}
  % = \frac{\revision{\mathcal{R}_1} \cdot (\sqrt{1+\rho} -
  % \frac{1}{\sqrt{\mathcal{A}}})
  % }{1-\frac{1}{\sqrt{\mathcal{A}}}}
  % \\
  % V_2' & = \frac{\revision{\mathcal{R}_1} (1+\rho)}{\revision{\mathcal{R}_2}} \cdot
  % \left(
  % \frac{r_2^\text{equiv}}{\sqrt{1+\rho}}
  % - \frac{\revision{\mathcal{R}_2}}{\sqrt{\mathcal{A}}-1}
  % \right)
  % \nonumber \\
  % & = \frac{
  % \revision{\mathcal{R}_1} \cdot (
  % \sqrt{1+\rho} -\frac{1+\rho}{\sqrt{\mathcal{A}}}
  % )
  % }{
  % 1-\frac{1}{\sqrt{\mathcal{A}}}
  % } 
  % \\
\end{align}

When $-1 \leq \rho \leq \frac{1}{\mathcal{A}} -1$, then token$_1$ becomes depleted, and the liquidity provider is left with token$_2$:
\begin{align}
  V' & = \frac{\revision{\mathcal{R}_1} (1+\rho)}{\revision{\mathcal{R}_2}} \cdot r'_2   =
  \revision{\mathcal{R}_1} \cdot (1+\rho) \cdot \left(\sqrt{\mathcal{A}} + 1 \right)
\end{align}

When $\rho \geq \mathcal{A} -1$, then token$_2$ becomes depleted, and the liquidity provider is left with token$_1$:
\begin{align}
  V' & = r'_1   =
  \revision{\mathcal{R}_1}  \cdot \left(\sqrt{\mathcal{A}} + 1 \right)
\end{align}


The divergence loss can thus be calculated as:
\begin{align}
  L(\rho) & = \frac{V'}{V_\text{held}} -1 \nonumber                                 \\
          & = \begin{cases}
                \frac{(\rho + 1) \cdot \sqrt{\mathcal{A}}  - 1}{2+\rho},
                 & -1 \leq \rho \leq \frac{1}{\mathcal{A}} -1
                \\
                \frac{\frac{\sqrt{1+\rho}
                  }{
                    1+\frac{\rho}{2}
                  } - 1
                }
                {1- \frac{1}{\sqrt{\mathcal{A}}}},
                 & \frac{1}{\mathcal{A}} -1 \leq \rho \leq \mathcal{A} -1
                \\
                \frac{\sqrt{\mathcal{A}}-1-\rho}{2+\rho},
                 & \rho \geq \mathcal{A} -1
              \end{cases}
  \label{eq:uniswapv3div}
\end{align}

Note that
$
  \lim_{\mathcal{A} \rightarrow 1} L(\mathcal{A} -1) =0
$.

\subsection{Balancer}


\subsubsection{Pool structure}

The Balancer protocol allows each liquidity pool to have more than 2 assets~\cite{martinelli2019whitepaper}. Each asset reserve $r_k$ is assigned with a weight $w_k$ at pool creation, where $\sum\limits_k w_k = 1$. Weights are pool hyperparameters, and do not change with either liquidity provision / removal or asset swap. The weight of an asset reserve represents the value of the reserve as a fraction of the pool value.

Balancer can be deemed a generalization of Uniswap; the latter is a special case of the former with $w_1 = w_2 = \frac{1}{2}$.

\subsubsection{Formulas}

\paragraph{Conservation function}

Balancer implements a conservation function with a weighted-product invariant (\autoref{fig:balcons}). Specifically, the product of reserve quantities each raised to the power of its weight stays constant with swapping:
\begin{align}
  \label{eq:balcons}
  \const = \prod_{k}r_k^{w_k}
\end{align}

\paragraph{Spot exchange rate} Given the quantity ratio $r_1 : r_2$ between token$_1$ and 2 and the implicit assumption on their value ratio $w_1 : w_2$, the price of token$_2$ denominated by token$_1$ can be expressed as:

\begin{equation}
  \label{eq:balancer}
  {_1E_2}  = \frac{r_1 \cdot w_2}{r_2 \cdot w_1}
\end{equation}


\paragraph{Swap amount}
We investigate the case when a user swaps token$_1$ for token$_2$, while the reserves of all other assets remain untouched in the pool.
Based on the Balancer conservation function (\autoref{eq:balcons}), the amount of token$_2$ received $x_2$ (spent when $x_2<0$) given amount of token$_1$ spent $x_1$ (received when $x_1<0$) can be calculated following the steps described in \autoref{sec:form_sa}:
\begin{align}
  \label{eq:balancerinput}
  r'_1 & = r_1 + x_1
  \nonumber                                                 \\
  r'_2 & = r_2\left(\frac{r_1}{r'_1}\right)^\frac{w_1}{w_2}
  \nonumber                                                 \\
  x_2  & = r_2 - r'_2
\end{align}


% \subparagraph{Input given output}

% \begin{align}
% \label{eq:balanceroutput}
% r'_2 &= r_2 - x_2
% \\
% r'_1 &= r_1\left(\frac{r_2}{r'_2}\right)^\frac{w_2}{w_1}
% \\
% x_1 &= r'_1 - r_1
% \end{align}

\paragraph{Slippage}

The slippage that a Balancer user experiences when swapping $x_1$ token$_1$ with $x_2$ token$_2$ can be expressed as:
\begin{align}
  S(x_1) = \frac{x_1/x_2}{{_1E_2}} -1 = \frac{
  \frac{x_1}{r_1} \cdot \frac{w_1}{w_2}
  }{
  1- \left(\frac{r_1}{r'_1}\right)^{\frac{w_1}{w_2}}
  }-1
  \label{eq:balancerslippage}
\end{align}

\autoref{fig:balancerslippage} illustrates the relationship between Uniswap slippage and normalized token$_1$ reserve change $\frac{x_1}{r_1}$.


\paragraph{Divergence loss}



Given the constant value ratio assumption with Balancer, the value of the entire pool $V$ can be expressed by the reserve quantity of token~1, $r_1$ divided by its weight $w_1$ (token$_1$ being numéraire):
\begin{align}
  V & =
  \frac{V_1}{w_1} =
  \frac{V_2}{w_2}
  = \frac{V_k}{w_k} = \frac{r_1}{w_1}
\end{align}
% \\
% V & = V_1 +V_2

If token$_2$ appreciates by $\rho$ (depreciates when $\rho<0$) while all other tokens' prices remain unchanged, the total value of the original reserve composition, when held outside of the pool, $V_\text{held}$ becomes:
\begin{align}
  V_\text{held} & = V + V_2 \cdot \rho
  = V \cdot (1+ w_2 \cdot \rho)
  % \frac{r_1 \cdot (1+ w_2 \cdot \rho)}{w_1} 
\end{align}

With $r_1$ token$_1$ and $r_2$ token$_2$ locked in a liquidity pool from the beginning, their quantity ratio would have been updated through users' swapping to result in token$_2$'s price change of $\rho$. The value ratio between the pool, token$_1$ and token$_2$, remains $1:w_1:w_2$, and the updated pool value $V'$ becomes:
\begin{align}
  V' & = \frac{V'_1}{w_1} =
  % \frac{V'_2}{w_2} = 
  \frac{r_1'}{w_1} =
  \frac{r_1 \cdot (1+ \rho)^{w_2}}{w_1}
  = V \cdot (1+ \rho)^{w_2}
\end{align}

The exchange rate range corresponds the liquidity provider's range requirement. Specifically, when $r'_2  = \frac{r_2}{(1+ \rho)^{1- w_2}}$
and
% $p' = \frac{(1+\rho) r_1 \cdot w_2}{r_2 \cdot w_1}$. 
% Furthermore, 
$r'_k = r_k \cdot (1+\rho)^{w_2}$ for $k\neq 2$, reflecting the assumed scenario that only the value of token$_2$ appreciates by $\rho$, while the value of all other tokens against token$_1$ remains unchanged.

As illustrated in \autoref{fig:balancerdiv}, the divergence loss due to liquidity provision as opposed to holding can thus be expressed as a function of price change:
\begin{align}
  L(\rho) & =
  \frac{V'}{V_\text{held}} -1 = \frac{(1+ \rho)^{w_2}}{1+w_2 \cdot \rho} -1
  \label{eq:balancerdiv}
\end{align}


\subsection{Curve}

\subsubsection{Pool structure}

With the Curve protocol, formerly StableSwap \cite{Egorov2019}, a liquidity pool consists of two or more assets with the same peg, for example, \coin{USDC} and \coin{DAI}, or \coin{wBTC} and \coin{renBTC}.


\subsubsection{Formulas}

\paragraph{Conservation function}
As assets from the same pool are connected to the same peg by design, the ideal exchange rate between them should always equal 1. Theoretically, this could be achieved by a constant-sum invariant. Nevertheless, Curve seeks to allow an exchange rate to deviate from 1, in order to reflect the supply-demand dynamic, while simultaneously keeping the slippage low.

Curve achieves this by interpolating between two invariants, constant sum and constant product \cite{Egorov2019}, with hyperparameter $\mathcal{A}$ as the interpolating factor (\autoref{eq:curvcons}).\footnote{Note that $\mathcal{A}$ here is equivalent to $A \cdot n^n$ in Curve's white paper \cite{Egorov2019}.} When $\mathcal{A} \rightarrow 0$, the conservation function boils down to a constant-product one, as with Uniswap; when $\mathcal{A} \rightarrow +\infty$, the conservation function is essentially a constant-sum one with constant exchange rate equal to 1 (\autoref{fig:curvcons}).
\begin{align}
  \label{eq:curvcons}
  \mathcal{A} \left(\tfrac{\sum\limits_k r_k}{\const}-1\right) & = \tfrac{
    \left(\frac{\const}{n}\right)^n
  }{\prod\limits_k r_k} -1
\end{align}

\paragraph{Spot exchange rate}

Rearrange \autoref{eq:curvcons} and let
\begin{align}
  Z(r_1,r_2)
  =
  \tfrac{
    \left(\frac{\const}{n}\right)^n
  }{r_1 r_2 \prod\limits_{k \neq 1,2} r_k} -1 - \mathcal{A} \left(\tfrac{r_1 + r_2 + \sum\limits_{k \neq 1,2} r_k}{\const}-1\right)
  \nonumber
\end{align}

Following \autoref{sec:genform}, the spot exchange rate can be calculated as:
\begin{align}
  _1E_2 = \tfrac{
    \partial Z(r_1,r_2)/\partial r_2
  }{
    \partial Z(r_1,r_2)/\partial r_1
  }
  = \tfrac{
    r_1 \cdot \left[\mathcal{A} \cdot r_2 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
  }{
    r_2 \cdot \left[\mathcal{A}  \cdot r_1 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
  }
  \label{eq:curvexchange}
\end{align}

% \begin{equation}
% \label{eq:balancer}
% p  = \frac{r_2 \cdot w_2}{r_2 \cdot w_1}
% \end{equation}

\paragraph{Swap amount}

We investigate the case when a user swaps token$_1$ for token$_2$, while the reserves of all other assets remain untouched in the pool.
Based on the Curve conservation function (\autoref{eq:curvcons}), the amount of token$_2$ received $x_2$ (spent when $x_2<0$) given amount of token$_1$ spent $x_1$ (received when $x_1<0$) can be calculated following the steps below:
\begin{align}
  \label{eq:curveinput}
  r'_1 & = r_1 + x_1
  \nonumber                                                                                                       \\
  r'_2 & = \tfrac{\sqrt{\frac{4 \const \left(\frac{\const}{n}\right)^n}{\mathcal{A} \cdot \prod\limits_{k\neq 2}'
      }+\left[\left(1-\frac{1}{\mathcal{A}}\right) \const -\sum\limits_{k\neq 2}'\right]^2}+\left(1-\frac{1}{\mathcal{A}}\right) \const - \sum\limits_{k\neq 2}'
  }{2}
  \nonumber                                                                                                       \\
  x_2  & = r_2 - r'_2
\end{align}

where
\begin{align}
  \prod\limits_{k\neq 2}' = r'_1 \cdot \prod\limits_{k \neq 1,2} r_k
  \quad \text{and} \quad
  \sum\limits_{k\neq 2}' = r'_1 + \sum\limits_{k \neq 1,2} r_k
\end{align}


\paragraph{Slippage}

As illustrated in \autoref{fig:curveslippage}, the slippage that a Curve user experiences when swapping $x_1$ token$_1$ with $x_2$ token$_2$ can be expressed as:
\begin{align}
  S(x_1) & = \tfrac{x_1/x_2}{_1E_2} -1
  \label{eq:curveslippage}
  \\
         &
  = \tfrac{
    \frac{
      x_1 \cdot \left[\mathcal{A}  \cdot r_1 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }{
      r_1 \cdot \left[\mathcal{A} \cdot r_2 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }
  }{1 -
    \frac{\sqrt{\frac{4 \const \left(\frac{\const}{n}\right)^n}{a \cdot \prod\limits_{k\neq 2}'
        }+\left[\left(1-\frac{1}{a}\right) \const -\sum\limits_{k\neq 2}'\right]^2}+\left(1-\frac{1}{a}\right) \const - \sum\limits_{k\neq 2}'
    }{2 r_2}
  }-1
  \nonumber
\end{align}


\paragraph{Divergence loss}

Curve's divergence loss in full form cannot be easily presented in a concise and comprehensible fashion.
Therefore, for Curve, we use the generalized method to calculate its divergence loss as described in \autoref{sec:genform}. The divergence loss in the case of a 2-asset pool is presented in \autoref{fig:curvediv}.


\subsection{DODO}

\subsubsection{Pool structure}

DODO only supports 2-asset liquidity pools at the moment. The pool creator opens a new pool with some amount of reserves on both sides, which determines the initial equilibrium state of the pool.

Importantly, the pool always anchors the exchange rate between the two assets to the external data fed by a price oracle. Thus, unlike Uniswap where asset exchange rates are implied by their reserve quantities, DODO allows the reserve ratio between the two assets within a pool to be arbitrary, while still maintaining the asset exchange rate close to the market rate. Due to this feature, DODO differentiates itself from traditional AMMs, and terms their pricing algorithm as ``Proactive Market Making" algorithm, or PMM.


\subsubsection{Formulas}

\paragraph{Spot exchange rate}

As presented in the previous sections, conventional AMMs derive the exchange rate between two assets in a pool purely from the conservation function. DODO does it the other way around: resorting to external market data as a major determinant of the exchange rate, DODO has its conservation function derived from its exchange rate formula.

The exchange rate between the two assets in a DODO pool is set by the market rate with an adjustment based on the pool composition.
We denote the market exchange rate as $P$, namely $1 \text{ token}_2 = P \text{ token}_1$, and the initial reserve for token$_1$ and token$_2$ as $\revision{\mathcal{R}_1}$ and $\revision{\mathcal{R}_2}$ respectively. The formula \autoref{eq:dodoexchange} sets the exchange rate $_1E_2$ higher than the market rate $P$---i.e. token$_2$ exhibits higher price in the pool than in the market, when the reserve of token$_1$ $r_1$ exceeds its initial state $\revision{\mathcal{R}_1}$, and sets $_1E_2$ lower than $P$---i.e. token$_1$ more expensive than its market value, when $r_1$ falls short of $\revision{\mathcal{R}_1}$. Formally,
\begin{align}
  \label{eq:dodoexchange}
  {_1E_2} & =
  \begin{cases}
    {P} \left[ 1 + \mathcal{A}\left( \left(\frac{\revision{\mathcal{R}_2}}{r_2}\right)^2-1\right) \right],         & r_1 \geq \revision{\mathcal{R}_1}
    \\
    {P} \Bigg/ \left[ 1 + \mathcal{A}\left( \left(\frac{\revision{\mathcal{R}_1}}{r_1}\right)^2-1\right) \right] , & r_1 \leq \revision{\mathcal{R}_1}
  \end{cases}
\end{align}


% \begin{align}
% \label{eq:DODOexchange}
% {_2E_1}  &= 
% \begin{cases}
% 1 \Bigg/  {P} \left[ 1 + \mathcal{A}\left( \left(\frac{\revision{\mathcal{R}_2}}{r_2}\right)^2-1\right) \right], & r_1 \geq \revision{\mathcal{R}_1} 
% \\
% \left[ 1 + \mathcal{A}\left( \left(\frac{\revision{\mathcal{R}_1}}{r_1}\right)^2-1\right) \right]\Bigg/  {P} , & r_1 \leq \revision{\mathcal{R}_1}
% \end{cases}
% \end{align}


\paragraph{Conservation function}

DODO's conservation function can be derived from its exchange formula \autoref{eq:dodoexchange}. In particular, the initial state of token$_1$ and token$_2$ reserves, $\revision{\mathcal{R}_1}$ and $\revision{\mathcal{R}_2}$ can be regarded as the two invariants of the conservation function.
This aligns with the definition according to our framework (\autoref{sec:formal}), as $\revision{\mathcal{R}_1}$ and $\revision{\mathcal{R}_2}$ remain constant with swapping activities, but get updated with liquidity provision or withdrawal.
\begin{align}
  \label{eq:dodocons}
       & r_1-\revision{\mathcal{R}_1}  = \int_{r_2}^{\revision{\mathcal{R}_2}}
  {P} \left[ 1 + \mathcal{A}\left( \left(\tfrac{\revision{\mathcal{R}_2}}{\delta}\right)^2-1\right) \right]
  \, d\delta
  \nonumber                                                                                                                                     \\
  = \, & P \cdot
  (\revision{\mathcal{R}_2} - r_2)
  \cdot \left[1 + \mathcal{A} \cdot \left(\tfrac{\revision{\mathcal{R}_2}}{r_2} -1 \right) \right],
  \quad r_1 \geq \revision{\mathcal{R}_1}                                                                                                       \\
       & r_2-\revision{\mathcal{R}_2}  = \int_{r_1}^{\revision{\mathcal{R}_1}}
  \frac{ 1 + \mathcal{A}\left( \left(\frac{\revision{\mathcal{R}_1}}{\delta}\right)^2-1\right) }
  {P}
  \, d\delta
  \nonumber                                                                                                                                     \\
  = \, & \frac{(\revision{\mathcal{R}_1} - r_1) \cdot \left[1 + \mathcal{A} \cdot \left(\frac{\revision{\mathcal{R}_1}}{r_1} -1 \right) \right]
  }{P}, \quad  r_1 \leq \revision{\mathcal{R}_1}
\end{align}

In the special case of $\mathcal{A} = 1$, when $C_1 = P \cdot C_2$, i.e. liquidity provided on both assets are of equal value, then DODO's conservation function is equivalent to Uniswap, with $r_1 \cdot r_2 = C_1 \cdot P \cdot C_2$. This can be observed from \autoref{fig:consfunc}, where the DODO's conservation function curve with $\mathcal{A} \rightarrow 1$ appears identical to that of Uniswap.


\paragraph{Swap amount}

The swap amount can be derived directly from the DODO conservation function (\autoref{eq:dodocons}):
% $x_1 > 0$
\begin{align}
   & r_1' = r_1 + x_1
  \nonumber
  \\
   & r_2' =
  % \nonumber
  % \\
  % &
  \begin{cases}
    \tfrac{
      {
          \revision{\mathcal{R}_1}- r_1'+ P \cdot \revision{\mathcal{R}_2} \cdot (1-2\mathcal{A}) +
          \atop
          \sqrt{
            \left[\revision{\mathcal{R}_1}-r_1' + P \cdot \revision{\mathcal{R}_2} \cdot (1-2\mathcal{A})\right]^2 + 4 \mathcal{A} \cdot (1-\mathcal{A}) \cdot (P \cdot \revision{\mathcal{R}_2})^2
          }
        }
    }{2 P \cdot (1- \mathcal{A})},
          & r_1' \geq \revision{\mathcal{R}_1} \\
    \revision{\mathcal{R}_2} + \frac{(\revision{\mathcal{R}_1} - r_1') \cdot \left[1 + \mathcal{A} \cdot \left(\frac{\revision{\mathcal{R}_1}}{r_1'} -1 \right) \right]
    }{P}, & r_1' \leq \revision{\mathcal{R}_1}
  \end{cases}
  \nonumber           \\
   & x_2 = r_2 - r_2'
  \label{eq:dodoswap}
\end{align}


% where $Q(r)$ is the difference between token$_2$'s target reserve quantity, $\revision{\mathcal{R}_2}$, and the amount of token$_2$ when token$_1$'s reserve quantity moves from $\revision{\mathcal{R}_1}$ to $r$. Formally,

% \begin{align}
% Q(r) = 
% \begin{cases}
% P \cdot (r-\revision{\mathcal{R}_1}) \cdot \left(1+\mathcal{A} \cdot \left(\frac{\revision{\mathcal{R}_1}}{r} -1 \right)\right), & r > \revision{\mathcal{R}_1} \\
% - \frac{
% P \cdot (r-\revision{\mathcal{R}_1}) + (1-2\mathcal{A}) \revision{\mathcal{R}_2} +
% \sqrt{
% \left(P \cdot (r-\revision{\mathcal{R}_1})
% \right)^2  + 2(1-2\mathcal{A}) \cdot P \cdot (r-\revision{\mathcal{R}_1}) \cdot \revision{\mathcal{R}_2} +  (\revision{\mathcal{R}_2})^2
% }
% }{2 (1- \mathcal{A})}, & r < \revision{\mathcal{R}_1}
% \\
% \frac{P \cdot (r-\revision{\mathcal{R}_1})}{
% \mathcal{A} \cdot \left[ \left(\frac{\revision{\mathcal{R}_1}}{r_1}\right)^2-1\right]}
% , & r < \revision{\mathcal{R}_1}
% \end{cases}
% \end{align}
% \frac{\sqrt{b^2 - 4ac}-b}{2a}, \text{where}\\
% \begin{cases}
% l \\ 
% f 
% \end{cases}
% \int_{r_1}^{r_1'} {_1E_2(r)} dr 
% = {P} x_1 \left[1 + \mathcal{A} \left( \frac{r_1^{\text{t}^2}}{r_1 r_1'}-1 \right) \right]
% \\
% x_1 &= \int_{r_2}^{r_2'} {_1E_2(r_2)} dr_2 = \frac{1}{P} \left(r_2' - r_2 \right) \left(1-\mathcal{A} + \mathcal{A} \frac{r_2^{\text{LP}^2}}{r_2 r_2'} \right)


\paragraph{Slippage}

As illustrated in \autoref{fig:dodolippage}, the slippage that a DODO user experiences when swapping $x_1$ token$_1$ with $x_2$ token$_2$ can be expressed as:

\begin{align}
  \label{eq:dodoslippage}
   & S(x_1) =
  \\
   &
  \begin{cases}
    \frac{2 \cdot (1-\mathcal{A}) \cdot x_1
    }{
      {r_1'-\revision{\mathcal{R}_1}+\revision{\mathcal{R}_2} \cdot P -
          \atop
          \sqrt{
            \left[\revision{\mathcal{R}_1}-r_1' + P \cdot \revision{\mathcal{R}_2} \cdot (1-2\mathcal{A})\right]^2 + 4 \mathcal{A} \cdot (1-\mathcal{A}) \cdot (P \cdot \revision{\mathcal{R}_2})^2
          }
        }
    } -1,
                                                                                                                                & r_1' \geq \revision{\mathcal{R}_1} \\
    \frac{x_1
    }{(r_1'-\revision{\mathcal{R}_1}) \cdot \left[1+A \cdot \left( \frac{\revision{\mathcal{R}_1}}{r_1'}-1 \right) \right]} -1, & r_1' \leq \revision{\mathcal{R}_1}
  \end{cases}
  \nonumber
\end{align}


\paragraph{Divergence loss}

DODO eliminates the kind of divergence loss seen in previously discussed protocols by not forcing liquidity providers to deposit tokens in pre-defined ratios. This is achieved by leveraging price oracles, which allow liquidity providers to deposit an arbitrary combination of base and quote tokens, unlocking single-token exposure. The price oracle is used to protect LPs against heavy arbitrage.



% First of all, we express the token$_1$ reserve quantity $R_1(x_1)$, 
%  pool value as a function of $r_1$'s quantity change, $x_1$. Specifically,


% \begin{align}
% R_1(x_1) &= r'_1 = r_1 + x_1x
% \\
% R_2(x_1) &= r'_2
% \\
% V(x_1) & = R_1(x_1) + R_2(x_1) \cdot P(x_1)
% \end{align}

% \begin{align}
% x_1 &= \chi(\rho)
% \\
% \rho &= \chi^{-1}(x_1) = \frac{p'}{p}-1 = \frac{P(x_1)}{P(0)}-1
% \\
% L(\rho) &= \frac{V(\chi(\rho))}{V(0)} -1
% \label{eq:curvediv}
% \end{align}

% Imperment loss is a function of price change...

% We express $x_1$, the amount needed to materalize the price change, as a function of $\rho$



\input{exhibits/consfunc}

\input{exhibits/slippage}

\input{exhibits/divloss}

==> backup/curve_old.tex <==
\begin{align}
\label{eq:curvcons}
\const = \mathcal{A} \cdot \sum\limits_k r_k + 
\ln \prod\limits_k r_k
\end{align}

\begin{align}
    _1E_2 = \frac{
    \partial Z(r_1,r_2)/\partial r_2
    }{
    \partial Z(r_1,r_2)/\partial r_1
    } 
    = \frac{
    r_1 \cdot \left(\mathcal{A} \cdot r_2 
    + 1 \right)
    }{
    r_2 \cdot \left(\mathcal{A}  \cdot r_1 + 1 \right)
    }
    \label{eq:curvexchange}
\end{align}

Curve achieves this by interpolating between two invariants, constant sum and constant product \cite{Egorov2019}, with hyperparameter $\mathcal{A}$ as the interpolating factor (\autoref{eq:curvcons}).\footnote{Note that $\mathcal{A}$ here is equivalent to $A \cdot n^n$ in Curve's white paper \cite{Egorov2019}.} When $\mathcal{A} \rightarrow 0$, the conservation function boils down to a constant-product one, as with Uniswap; when $\mathcal{A} \rightarrow +\infty$, the conservation function is essentially a constant-sum one with constant exchange rate equal to 1 (\autoref{fig:curvcons}).


\begin{align}
\label{eq:curvcons}
\mathcal{A} \left(\frac{\sum\limits_k r_k}{\const}-1\right) &= \frac{
\left(\frac{\const}{n}\right)^n
}{\prod\limits_k r_k} -1
\end{align}



\paragraph{Spot exchange rate}

Rearrange \autoref{eq:curvcons} and let
\begin{align}
    Z(r_1,r_2) & = \frac{
\left(\frac{\const}{n}\right)^n
}{r_1 r_2 \prod\limits_{k \neq 1,2} r_k} -1 - \mathcal{A} \left(\frac{r_1 + r_2 + \sum\limits_{k \neq 1,2} r_k}{\const}-1\right)
\end{align}

Following \autoref{sec:genform}, the spot exchange rate can be calculated as:


\begin{align}
    _1E_2 = \frac{
    \partial Z(r_1,r_2)/\partial r_2
    }{
    \partial Z(r_1,r_2)/\partial r_1
    } 
    = \frac{
    r_1 \cdot \left[\mathcal{A} \cdot r_2 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }{
    r_2 \cdot \left[\mathcal{A}  \cdot r_1 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }
    \label{eq:curvexchange}
\end{align}

% \begin{equation}
% \label{eq:balancer}
% p  = \frac{r_2 \cdot w_2}{r_2 \cdot w_1}
% \end{equation}

\paragraph{Swap amount}

We investigate the case when a user swaps token$_1$ for token$_2$, while the reserves of all other assets remain untouched in the pool.
Based on the Curve conservation function (\autoref{eq:curvcons}), the amount of token$_2$ received $x_2$ (spent when $x_2<0$) given amount of token$_1$ spent $x_1$ (received when $x_1<0$) can be calculated following the steps below:


\begin{align}
\label{eq:curveinput}
r'_1 &= r_1 + x_1
\nonumber \\
r'_2 &= \frac{\sqrt{\frac{4 \const \left(\frac{\const}{n}\right)^n}{\mathcal{A} \cdot \prod\limits_{k\neq 2}'
}+\left[\left(1-\frac{1}{\mathcal{A}}\right) \const -\sum\limits_{k\neq 2}'\right]^2}+\left(1-\frac{1}{\mathcal{A}}\right) \const - \sum\limits_{k\neq 2}'
}{2}
\nonumber \\
x_2 &= r_2 - r'_2
\end{align}

where 

\begin{align}
\prod\limits_{k\neq 2}' &= r'_1 \cdot \prod\limits_{k \neq 1,2} r_k \\
\sum\limits_{k\neq 2}' &= r'_1 + \sum\limits_{k \neq 1,2} r_k
\end{align}

% \subparagraph{Input given output}

% \begin{align}
% x_2 &= r_2 - r'_2
% \\
% r'_1 &= \frac{\sqrt{\frac{4 \const \left(\frac{\const}{n}\right)^n}{a \cdot \prod\limits_{k\neq 1}'
% }+\left[\left(1-\frac{1}{a}\right) \const -\sum\limits_{k\neq 1}'\right]^2}+\left(1-\frac{1}{a}\right) \const - \sum\limits_{k\neq 1}'
% }{2}
% \\
% x_1 &= r'_1 - r_1
% \label{eq:uniswapoutput}
% \end{align}

% where 

% \begin{align}
% \prod\limits_{k\neq 1}' &= r'_2 \cdot \prod\limits_{k \neq 1,2} r_k \\
% \sum\limits_{k\neq 1}' &= r'_2 + \sum\limits_{k \neq 1,2} r_k
% \end{align}


\paragraph{Slippage}

As illustrated in \autoref{fig:curveslippage}, the slippage that a Curve user experiences when swapping $x_1$ token$_1$ with $x_2$ token$_2$ can be expressed as:

\begin{align}
S(x_1) & = \frac{x_1/x_2}{_1E_2} -1 
\\
& = \frac{
\frac{
x_1 \cdot \left[\mathcal{A}  \cdot r_1 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }{
    r_1 \cdot \left[\mathcal{A} \cdot r_2 \cdot \prod\limits_k r_k + \const \cdot \left(\frac{\const}{n}\right)^n\right]
    }
}{1 - 
\frac{\sqrt{\frac{4 \const \left(\frac{\const}{n}\right)^n}{a \cdot \prod\limits_{k\neq 2}'
}+\left[\left(1-\frac{1}{a}\right) \const -\sum\limits_{k\neq 2}'\right]^2}+\left(1-\frac{1}{a}\right) \const - \sum\limits_{k\neq 2}'
}{2 r_2}
}-1
\label{eq:curveslippage}
\end{align}


\paragraph{Divergence loss}

Curve's divergence loss in full form cannot be easily presented in a concise and comprehensible fashion. 
Therefore, for Curve, we use the generalized method to calculate it's divergence loss as described in \autoref{sec:genform}. The divergence loss in the case of a 2-asset pool is presented in \autoref{fig:curvediv}.

==> exhibits/security_exhibit.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/securityTaxonomy.pdf}
    \caption{Taxonomy of DeFi Security}
    \label{fig:security}
\end{figure}

==> exhibits/volume_poolcount.tex <==
\begin{figure}[tbh]
    \centering
    \begin{subfigure}[b]{0.43\linewidth}
        \centering
        \includegraphics[height=0.085\paperheight, trim={0 0 0 0},clip]{figures/volume_and_poolcount_uniswap.pdf}
        \caption[Uniswap V2]%
        {{\small Uniswap V2}}
        \label{fig:uniswap_vol_poolcount}
    \end{subfigure}
    \begin{subfigure}[b]{0.43\linewidth}
        \centering
        \includegraphics[height=0.085\paperheight, trim={0 0 0 0},clip]{figures/volume_and_poolcount_balancer.pdf}
        \caption[Balancer]%
        {{\small Balancer}}
        \label{fig:balancer_vol_poolcount}
    \end{subfigure}
    \begin{subfigure}[b]{0.43\linewidth}  \centering
        \includegraphics[height=0.085\paperheight, trim={0 0 0 0},clip]{figures/volume_and_poolcount_curve.pdf}
        \caption[Curve]%
        {{\small Curve}}
        \label{fig:curve_vol_poolcount}
    \end{subfigure}
    \begin{subfigure}[b]{0.43\linewidth}
        \centering
        \includegraphics[height=0.085\paperheight, trim={0 0 0 0},clip]{figures/volume_and_poolcount_dodo.pdf}
        \caption[DODO]%
        {{\small DODO}}
        \label{fig:Dodo}
    \end{subfigure}
    \caption[ caption ]
    {\small Monthly volume (blue bars) and the total pool count (red line) for AMMs. Data from \href{https://thegraph.com/explorer/}{The Graph} and \href{https://duneanalytics.com/hagaetc/dex-metrics}{Dune Analytics}.}
    \label{fig:pooltimeseries}
\end{figure}

==> sections/futureresearch.tex <==
\subsection{Avenue of future research}
\input{exhibits/landscape_table}

==> sections/pastevents.tex <==
\section{Past security exploits}
\label{sec:pastevent}

% https://insights.glassnode.com/defi-attacks-flash-loans-centralized-price-oracles/
% https://messari.io/article/exploiting-defi-apps-with-this-one-weird-trick
% https://blog.chain.link/flash-loans-and-the-importance-of-tamper-proof-oracles/


% Flash loan funded price oracle attacks: use flash loans to exploit vulnerabilities in centralized price oracles, manipulate asset's prices and siphon funds from contracts. 

% Examples: 

% Harvest finance: https://news.bitcoin.com/defi-protocol-harvest-finance-hacked-for-24-million-attacker-returns-2-5-million/
% Value Defi: https://blog.peckshield.com/2020/11/15/valuedefi/
% Cheese bank: https://peckshield.medium.com/cheese-bank-incident-root-cause-analysis-d076bf87a1e7


% Attack of uniswap pool (not related to price oracle): https://defirate.com/imbtc-uniswap-hack/










\begin{enumerate}
    \item A user takes out a flash loan to borrow a large amount of token A from a PLF as Aave for example.
    \item That user now swaps token A for token B on a \ac{dex}, causing a price decrease in token A and a price increase in token B, thus actively manipulating price. Huge trading amounts are possible through the use of big flash loan amounts.
    \item That manipulated price is now the source of truth for protocols that use a DEX as their sole price oracle, which harms the ecosystem markets. If the vulnerable protocol for example is a PLF, using token B as temporary collateral allows the user to borrow a larger amount of token A than should normally be possible.
    \item A portion of token A is than used to pay back the flash loan
    \item The remaining tokens are profits for the flash loan user.
\end{enumerate}




==> sections/security.tex <==
\section{Security and privacy issues with AMM}
\label{sec:security}

\subsection{Definitions}

\textbf{Miner Extractable Value}
Philip Daian and co-authors defined the MEV as "value that is extractable by miners directly from smart
contracts as cryptocurrency profits" in their Flash Boys 2.0 paper. However, this definition no longer captures all the activity. In fact, the acronym MEV, changed its first word, MEV now stands for Maximum Extractable Value.

\textbf{Maximum Extractable Value}: includes the above activities and  extends to include the mined transactions that bypass the mempool and are immediately mined without being broadcasted.

From this point onwards, unless explicitly stated, MEV is to stand for \textbf{Maximum Extrctable Value}.

A quote from the Flashbots website\footnote{https://explore.flashbots.net/faq} higlights the distinction further

\begin{displayquote}

    \[ . . . \]

    \text{[...]} MEV exists on all smart contract blockchains where there is a party responsible for transaction ordering, including non-miner actors such as validators in ETH2.0 and rollup providers on Optimistic Rollups. Therefore we propose to rename MEV as maximal extractable value, broadening the scope to cover other blockchain architectures, while still being ‘backwards compatible’ with its initial name (ie. hinting at the upper bound set by the rights of the most powerful actor with respect to transaction ordering).
\end{displayquote}

\textbf{MEV-miner}: miner that runs a modified Ethereum peer node client software. This enables extractors to privately relay their transactions bypassing the mempool.

\textbf{Extractor}: Code that utilises miners' \textbf{MEV-clients} to avoid broadcasting the transaction into the mempool. By routing the transaction directly to the \textbf{MEV-miner}, if there is enough hashpower, the block will be mined with \textbf{extractor's} transaction at zero gas fees. \textbf{Extractors} will pay the \textbf{MEV-miner} fee for such a service out of their profits. This is a transaction business lane to avoid mingling with the common folk.

\subsubsection{Agents' Privacy}
\textbf{Private agents}
The ones that have been working on proprietary software and have built working relationships with the miners. It is difficult to idnetify these agents, but their addresses are public domain knowledge and can be analysed.

\textbf{Public agents}
Flashbots. These work to democratise the MEV battlelines. Independent developers can team up to battle the rooted centralised private agents using these tools. The downside, of course, is that the private agents will have access to everything that these agents develop. Flashbots wrote open-sourced MEV-client\footnote{https://github.com/flashbots} library that would be ran by miners. Public agents would change their Ethereum provider to miners that use this modified geth client.


\subsection{\ac{amm} MEV attack vectors}

Some of the attacks herein do not only pertain to MEV, such as front-running. However, it is clear that zero gas fees let MEV traders transact more often and earn more, thus squeezing out the non-MEV traders out of the DEXes.



\section{MEV quantification}

The dashboard does not track multi-txn MEV. It tracks single transaction arbitrage and liquidation events. The pie charts below are taken from the website\footnote{https://explore.flashbots.net}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.42\linewidth}
        \centering
        \includegraphics[height=0.14\paperheight, trim={0 0 0 0},clip]{figures/mev-by-source.png}
        \caption[MEV by source]%
        {{\small MEV by source}}
        \label{fig:mev-by-source}
    \end{subfigure}
    \begin{subfigure}[b]{0.42\linewidth}
        \centering
        \includegraphics[height=0.14\paperheight, trim={0 0 0 0},clip]{figures/mev-by-type.png}
        \caption[MEV by type]%
        {{\small MEV by type}}
        \label{fig:mev-by-type}
    \end{subfigure}
    \\ \vskip 0.25cm
    \begin{subfigure}[b]{0.35\linewidth}  \centering
        \includegraphics[height=0.14\paperheight, trim={0 0 0 0},clip]{figures/mev-by-role.png}
        \caption[MEV by role]%
        {{\small MEV by role}}
        \label{fig:mev-by-role}
    \end{subfigure}
    \caption[ caption ]
    {\small MEV by (a) source, (b) type and (c) role}
    \label{fig:pooltimeseries}
\end{figure}



\section{Scams (find a better word)}

\subsubsection{Rug pulls}

Ramifi.org

\noindent https://info.uniswap.org/pair/0x3Fa4aEF6Fbf12f1c4b8593eca8c20ab2dD75f763

\noindent

quantify such scams

\section{Yield scams}

GOLD example

Websites like zapper.fi allow users to quickly identify lucrative yield opportunities. Very often the most degen APYs are scams. Talk about basis gold here.

\input{exhibits/security_exhibit}


something about the rug pulls input after this
The profit for the malicious user amounts to \\
$x_A \cdot (\frac{x_B}{x_B - \Delta} - 1)$.

https://etherscan.io/tx/0xe79515f4a14c84c64758a41d10db9cc94c66cfe0c63c476b408591bd810a813c

Nonce of the transaction in the block is 1! Meaning it is the second transaction, straight after the unlock of trading in Uniswap. And the gas fee? 30 gwei, and that's when the average gwei was 200 (confirm). We have observed that generally Polkastarter IDOs after the private sales, get listed on the Uniswap and get sniped by MEV bots french toasters. If there is no lock up on the privately sold tokens, these get dumped by the team and advisors on the just MEV pumped coin price. This creates a vicious cycle. More listings > private sales > attracts MEV bots > team dumps. The only agents benefiting here are (i) miners; (ii) MEV bots; (iii) token team. The trader made xxx in 10 minutes of trading.


By formalizing the mechanisms and recognizing these are generalizable for major \ac{amm} protocols, we divided the workings of \ac{amm} protocols in a generalized component and a differentiation component. Using the state space representation and generalized \ac{amm} formulas, an applicable \ac{amm} framework was built.
